KGNv2: Separating Scale and Pose Prediction for Keypoint-based 6-DoF Grasp Synthesis on RGB-D input

We propose a new 6-DoF grasp pose synthesis approach from 2D/2.5D input based on keypoints. Keypoint-based grasp detector from image input has demonstrated promising results in the previous study, where the additional visual information provided by color images compensates for the noisy depth perception. However, it relies heavily on accurately predicting the location of keypoints in the image space. In this paper, we devise a new grasp generation network that reduces the dependency on precise keypoint estimation. Given an RGB-D input, our network estimates both the grasp pose from keypoint detection as well as scale towards the camera. We further re-design the keypoint output space in order to mitigate the negative impact of keypoint prediction noise to Perspective-n-Point (PnP) algorithm. Experiments show that the proposed method outperforms the baseline by a large margin, validating the efficacy of our approach. Finally, despite trained on simple synthetic objects, our method demonstrate sim-to-real capacity by showing competitive results in real-world robot experiments.

==> intro.tex <==
\section{Introduction}\label{sec:Intro}

% The pipeline: Generate, evaluate, and optionally refinement. Emphasis the importance of generating diverse and accurate grasp candidates
Determining grasp configurations from visual sensor input is a
fundamental problem in robot manipulation. While great progress has been
made on the detection of top-down grasps using deep learning
\cite{dexnet22017, deepgrasp2018, gknet2021}, general purpose object
grasping requires 6-DoF grasp poses for task completion purposes or for
more flexibility in challenging situations. 

A typical 6-DoF grasp system involves 
a \textit{grasp generation} module for generating grasp candidates 
and a \textit{grasp evaluation} module for ranking the candidates
  regarding successful executability based on 
estimated grasp quality \cite{GeoEval2018}, 
collision considerations \cite{collision2021, implicitCollision2021}, 
or 
environemental constraints \cite{humanHandover2021, graspInPrinter2021}.
%
Some methods include a \textit{grasp pose refinement} module to
enhance the grasp success probability \cite{refineScore2017},
which can be interpreted as an iterative approach to the basic
process. 
Being the first step, a good \textit{grasp generation} algorithm
is a prerequisite for robust grasping.
An ideal grasp candidate set should contain poses that are
accurate and diverse to ensure functionality and flexibility in
constrained environments.


% People are using the point cloud. but the data is unordered, makes extracting the geometric information from it slow, limit the input point number, and usage.
Since 6-DoF grasp detection task requires 3D geometric reasoning, the
majority of approaces process 3D data.  The advent of deep point cloud
feature extractors, such as PointNet \cite{Pointnet2017} and PointNet++
\cite{Pointnet++2017}, has promoted investigation into grasp detection
from point cloud input \cite{pointnetGPD2019, 6dofGraspNet2019, s4g2020,%
GDN2020, pointnet++grasp2020, ContactGraspNet2021}.
The point cloud is preferable due to its more immediate
accessibility compared to other 3D data formats (e.g., meshes, voxels).
However, the geometric information is veiled since point clouds
are unordered.  Lost structure must be extracted using methods
such as hierarchical grouping and/or geometry-based sampling 
\cite{Pointnet++2017}. 
Empirically, point clouds have poor scaling; computational
cost soars as the input cardinality increases \cite{Randla-net2020}.
Consequently, point cloud grasp detection approaches require further
preprocessing to limit point cloud cardinality. 
Methods include segmentation \cite{6dofGraspNet2019, pointnetGPD2019} 
and downsampling \cite{s4g2020}, which may introduce segmentation 
error \cite{ContactGraspNet2021} or discard critical information.
In addition, point cloud methods could produce biased results due to
imbalanced point distributions.  Observations in \S\ref{sec:visResults}
show that small objects tend to be ignored.


% Here we focus on grasp generation from the RGB-D input.
\paragraph{Contribution}
In contrast, this paper explores 6-DoF grasp generation from monocular RGB-D
(2.5D) input.  
It proposes \textbf{a new single-view grasp generation method, named
\textit{\netName (\netNameS)},} inspired by object pose estimation
research \cite{perspectiveNet2019, centerPose2022} and advances in
top-down {\SE2} grasping \cite{gknet2021}.  The method first uses a
convolutional neural network (CNN) to detect the 2D perspective
projection of a set of predefined 3D keypoints in the gripper frame.  A
Perspective-n-Point (\PnP) algorithm then recovers the 3D grasp poses
from established 2D-3D correspondences.
% ADD IN IF ROOM:
% and camera intrinsics.

% Data
\textbf{To generate sufficiently rich and dense training data, we
construct a primitive shape dataset with continuously parameterized and
densely sampled grasp families}. The tactic leverages the simple,
closed-form nature of primitive object geometry to simplify
specification of the feasible grasp pose distribution.  
Once the distribution is defined, sampling involves generating a uniform
cover of the feasible grasp set. This overcomes the sampling
insufficiency of randomized sampling methods and related sample-based
grasp labeling strategies applied to arbitrary objects
\cite{sampleInvest}. 
Using primitive shapes also provides a principled way to evaluate both
accuracy and diversity of the predicted set.  
While primitive shapes may seem limiting, PS-CNN \cite{ps2022} observed
that common household objects are similar to primitive shapes or contain
primitive shape parts.  PS-CNN achieves top 6-DOF grasping performance by
recognizing primitive shape regions. Its drawback is a time-consuming 3D
model fitting process for dense grasp generation.  
Based on these findings, we conjecture that models trained on primitive
shape datasets can extrapolate to realistic objects, which is supported
by physical experiment outcomes in \S \ref{sec:phyExp}.

% Advantage of our method.
Testing shows that {\netNameS}, trained only on single primitive shape
data with a coarse covering of the grasp families, can ``fill in'' the
grasp pose gaps and achieves competitive performance.
Specifically, \textbf{{\netNameS} outperforms baselines on a single-object
test set, and achieves comparable results on a multi-object test set to a
baseline specifically trained for cluttered environments.}
It is more than 3-times faster than all baselines, and demonstrates
a significant advantage on small objects compared to point cloud
methods.  Again, physical experiments verify the transferability of the
approach to the embodied, real-world setting.





==> tables/tabPhyMulti.tex <==
\begin{table}[t!]
  \vspace*{-0.0in}
  \centering
  
%  \setlength\tabcolsep{5pt} 
  \renewcommand{\arraystretch}{1.1}
    \caption{Multi-object Physical Experiment Results}
  \begin{threeparttable}
  \begin{tabular}{|c| c c | c c |}
  		\hline
	Trail ID & Attempts & Success & Success Rate & Clear Rate \\
 		\hline
 	1 & 5 & 5 & 100\% & 100\%  \\
 	2 & 6 & 5 & 83.3\% & 100\%  \\
 	3 & 7 & 5 & 71.4\% & 100\%  \\
 	4 & 6 & 5 & 83.3\% & 100\%  \\
 	5 & 5 & 5 & 100\% & 100\%  \\
 	6 & 5 & 5 & 100\% & 100\%  \\
 	7 & 7 & 3 & 42.9\% & 60\%  \\
 	8 & 6 & 5 & 83.3\% & 100\%  \\
 	9 & 5 & 5 & 100\% & 100\%  \\
 	10 & 8 & 5 & 62.5\% & 100\%  \\
% 		\hhline{|======|}
		\hline\hline
 	Avg & 6.0 & 4.8 
 	& 80\%\tnote{${}^\star$} $\pm$ 10.1\% 
 	& 96\% $\pm$ 7.4\% 
 	\\
		\hline
  \end{tabular}
  \begin{tablenotes}
	  \item ${}^\star$ Calculated as the average success number over average attempts number.
  \end{tablenotes}
  \end{threeparttable}
  
  \label{tab:phyMulti}
  \vspace*{-0.2in}
\end{table}




==> tables/tabPhySingle.tex <==
\begin{table}[t!]
  \vspace*{-0.0in}
  \centering
  
%  \setlength\tabcolsep{5pt} 
  \renewcommand{\arraystretch}{1.25}
    \caption{Single-object Physical Experiment Results}
  \begin{threeparttable}
  \begin{tabular}{|c| c c | c | c c |}
  		\hline
	Object & KGN & \netName & Object & KGN & \netName \\
 		\hline
 	Ball & 4/5 & 4/5 & Cable & 5/5 & 5/5 \\
 	Tape & 5/5 & 5/5 & Box & 5/5 & 4/5 \\
 	Bowl & 4/5 & 5/5 & Mug & 4/5 & 5/5 \\
 	ToothBrush & 5/5 & 5/5 & Clamp & 3/5 & 4/5 \\
% 		\hhline{|======|}
		\hline\hline
 	\multicolumn{6}{|c|}{Mean} \\
 		\hline
 	KGN & \multicolumn{2}{c|}{87.5\% $\pm$ 9.6\%} & \textbf{\netName} & \multicolumn{2}{c|}{92.5\% $\pm$ 6.7\%}  \\
		\hline
  \end{tabular}
  \end{threeparttable}
  \label{tab:phySingle}
  \vspace*{-0.2in}
\end{table}


